Visualising interactive inferences with IDPD3

A large part of the use of knowledge base systems is the interpretation of the output by the end-users and the interaction with these users. Even during the development process visualisations can be a great help to the developer. We created IDPD3 as a library to visualise models of logic theories. IDPD3 is a new version of $ID^{P}_{Draw}$ and adds support for visualised interactive simulations.

==> idp-latex/idp-latex.tex <==
%IMPORTANT: ONLY INCLUDE AS \input{idp-latex/idp-latex}
\usepackage{import}

\subimport{idp-latex/}{includes-no-theorems}
\subimport{idp-latex/}{common-citations}
\subimport{idp-latex/}{theorems}


==> idp-latex/theorems.tex <==
\usepackage{amsthm}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem*{lem*}{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{lemma}[thm]{Lemma}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}

\newtheorem{nota}[thm]{Notation}
\newtheorem*{nota*}{Notation}


\newtheoremstyle{example_basic} 
{\topsep} %ABOVESPACE
{\topsep} %BELOWSPACE 
{\normalfont}% Body font 
{0pt}% Indent amount (empty = no indent, \parindent = para indent) 
{\bfseries}% Thm head font 
{.}% Punctuation after thm head 
{5pt plus 1pt minus 1pt}% Space after thm head (\newline = linebreak) 
{}% Thm head spec

\newtheoremstyle{example_contd}
{\topsep} %ABOVESPACE
{\topsep} %BELOWSPACE 
{\normalfont}% Body font 
{0pt}% Indent amount (empty = no indent, \parindent = para indent) 
{\bfseries}% Thm head font 
{.}% Punctuation after thm head 
{5pt plus 1pt minus 1pt}% Space after thm head (\newline = linebreak) 
{\thmname{#1} \thmnumber{ #2}\thmnote{#3} (continued)}% Thm head spec 

\theoremstyle{example_basic} 
\newtheorem{ex}[thm]{Example}
\newtheorem{example}[thm]{Example}
\newtheorem{remark}[thm]{Remark}

\newtheorem{ex*}{Example}
\theoremstyle{example_contd} 
\newtheorem*{ex_continued}{Example}

\theoremstyle{plain}



